Tree-Algorithms with Multi-Packet Reception and Successive Interference Cancellation

In this paper, we perform a thorough analysis of tree-algorithms with multi-packet reception (MPR) and successive interference cancellation (SIC), showing a number of novel results. We first derive the basic performance parameters, which are the expected length of the collision resolution interval and the normalized throughput, conditioned on the number of contending users. We then study their asymptotic behaviour, identifying an oscillatory component that amplifies with the increase in MPR. In the next step, we derive the throughput for the gated and windowed access, assuming Poisson arrivals. We show that for windowed access, the bound on maximum stable normalized throughput increases with the increase in MPR. his implies that investing in advanced physical capabilities, i.e., MPR and SIC pays off from the perspective of the medium access control algorithm.

==> B_K_figure.tex <==
% This file was created by tikzplotlib v0.9.8.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={$K$},
xmin=-3.95, xmax=104.95,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={$| B ( K, 1 ) |$},
scaled y ticks = false,
ymin=-0.00404208424334393, ymax=0.0848837691102225,
ytick style={color=black},
ytick={-0.01,0,0.01,0.02,0.03,0.04,0.05,0.06,0.07,0.08,0.09},
yticklabels={−0.01,0.00,0.01,0.02,0.03,0.04,0.05,0.06,0.07,0.08,0.09}
]
\path [draw=red, semithick, dash pattern=on 5.55pt off 2.4pt]
(axis cs:41,0)
--(axis cs:41,0.0808416848668786);

\addplot [semithick, color0]
table {%
1 4.47998480049241e-05
2 0.000204280864146624
3 0.000632094986513863
4 0.00150885086564667
5 0.00298994938036167
6 0.0051587856873903
7 0.00801127258752646
8 0.0114690482690359
9 0.0154068103799626
10 0.0196803024370502
11 0.0241477406887521
12 0.0286829716314185
13 0.0331816117669617
14 0.0375623360028562
15 0.0417653205397086
16 0.0457493193275903
17 0.0494883200013663
18 0.0529683133650653
19 0.056184434283347
20 0.0591385645492539
21 0.0618373964089597
22 0.0642909110373451
23 0.0665112095966036
24 0.0685116327931339
25 0.0703061103510052
26 0.0719086901456997
27 0.0733332055487022
28 0.074593047689972
29 0.0757010163963305
30 0.0766692294116738
31 0.0775090742250713
32 0.0782311905717046
33 0.0788454745931906
34 0.0793610979035164
35 0.0797865365406085
36 0.0801296061051471
37 0.0803975003899076
38 0.0805968315581453
39 0.0807336704960222
40 0.0808135863866773
41 0.0808416848668786
42 0.0808226443578699
43 0.0807607503303527
44 0.0806599273850187
45 0.080523769116447
46 0.0803555657884255
47 0.080158329889601
48 0.0799348196649121
49 0.0796875607343479
50 0.0794188659190912
51 0.0791308533982125
52 0.0788254633183883
53 0.0785044729758277
54 0.0781695106845863
55 0.077822068439381
56 0.0774635134743564
57 0.0770950988123477
58 0.0767179728922521
59 0.0763331883553545
60 0.0759417100649368
61 0.0755444224273215
62 0.0751421360766944
63 0.0747355939806313
64 0.0743254770182349
65 0.0739124090781536
66 0.073496961719496
67 0.0730796584347535
68 0.0726609785502787
69 0.0722413607966132
70 0.071821206577999
71 0.0714008829677152
72 0.0709807254534317
73 0.0705610404545569
74 0.0701421076315368
75 0.0697241820052398
76 0.0693074959029043
77 0.0688922607456278
78 0.0684786686910153
79 0.0680668941433739
80 0.0676570951427234
81 0.0672494146428842
82 0.0668439816879815
83 0.0664409124958806
84 0.066040311456307
85 0.0656422720507268
86 0.0652468777004405
87 0.0648542025487774
88 0.0644643121827708
89 0.0640772642992268
90 0.0636931093196763
91 0.0633118909583177
92 0.0629336467467077
93 0.0625584085186389
94 0.0621862028583546
95 0.0618170515149858
96 0.0614509717858567
97 0.0610879768710853
98 0.0607280762017042
99 0.0603712757433467
100 0.0600175782773753
};
\end{axis}

\end{tikzpicture}


==> d_ary.tex <==
\section{Remarks on $\tf$-ary Tree Algorithms with \ac{SIC}}
\label{sec:d-ary}

As discussed in Section~\ref{sec:TA}, $\tf$-ary tree algorithms (i.e., tree-algorithms in which the number of groups in which users can split is generalized to $\tf$)\footnote{From now on, we will refer to $\tf$ as the splitting factor}, show benefits in the original scenario (i.e., without SIC and MPR).
In particular, it was shown that the ternary version of the algorithm (i.e., when $d=3$) with optimized splitting probabilities outperforms the binary version.
A natural question is whether analogous results can be established for the variant of tree algorithms examined in this paper.

In this respect, the analysis presented in \cite[Section IV-A]{SICTA} is performed for $\tf$-ary tree algorithms with \ac{SIC} when $\mpr=1$.
However, the initial premise of the analysis is incorrect when $d > 2$. % rendering the corresponding results incorrect as well.
The premise states the following (verbatim):
\begin{align}
\label{eq:d-ary_wrong}
    \cri_\nuser = \begin{cases} 1, & \text{if } n = 0,1 \\
    \sum_{j=i}^d \cri_{I_j} , & \text{if } n \geq 2
    \end{cases}
\end{align}
where $I_j$ is the number of users selecting $j$-th group, $j \in \{ 1, 2, \dots, d\}$.
We illustrate its shortcomings through a simple example depicted in Fig.~\ref{fig:d-ary}a), in which we assume $d=3$, $\nuser = 2$ (and $\mpr =1$).
In slot 2, the receiver is able to decode the transmission occurring in it, and, after applying \ac{SIC}, recover the remaining transmission in slot 1.
As these two transmissions are the only ones, there is no need for further splitting, and the total duration of the \ac{CRI} is 2 slots.
However, according to \eqref{eq:d-ary_wrong}, the \ac{CRI} length in this example should be
\begin{align}
    l_2 = l_1 + l_1 + l_0 = 3.
\end{align}
In fact, if $\nuser=2$ and the first group has a single user, like in the Fig.~\ref{fig:d-ary}a), the length of the CRI will be 2 slots, irrespective of the value of the splitting factor $\tf$ (given that $\tf \geq 2$).
On the other hand, the example in Fig.~\ref{fig:d-ary}b) shows the case when the \ac{CRI} length is indeed 3 slots and agrees with the formula \eqref{eq:d-ary_wrong}.
In effect, the elegant conclusion drawn in \cite{SICTA} (verbatim)
\begin{align}
    (d-1) ( \ecri'_\nuser - 1) = d ( \ecri_\nuser - 1 )
\end{align}
where $\ecri'_\nuser$ is the expected conditional length of the \ac{CRI} for the standard tree algorithm (STA), does not hold in general for $d > 2$, also invalidating the subsequent throughput analysis that exploited the results known for the STA.

\begin{figure}[t]
  % Requires \usepackage{graphicx}
  \centering
  \includegraphics[width=0.4\columnwidth]{d-ary}
  %\includegraphics[width=0.6\columnwidth]{d-ary}
  \caption{Example of ternary splitting with \ac{SIC}, $\mpr = 1$.}
  \label{fig:d-ary}
\end{figure}

Generalizing the insights shown in Fig.~\ref{fig:d-ary}, for $\mpr=1$ we write
\begin{align}
\label{eq:dary_correct}
    \cri_\nuser = \begin{cases} 1, &  n = 0,1 \\
    \sum_{j=i}^{d_\text{min}} \cri_{I_j} , &  n \geq 2  
    \end{cases}
\end{align}
where $d_\text{min}$ is the minimum value of $o \in \{1,\dots, d\}$ for which the following holds
\begin{align}
\sum_{j=1}^{o} I_j \geq \nuser - 1.
\end{align}
The explanation of \eqref{eq:dary_correct} is intuitively clear -- the splitting process will stop as soon as there is a single user remaining from the original collision, no matter how many groups are left.

Generalizing \eqref{eq:dary_correct} for the case with \ac{MPR}, we obtain
\begin{align}
 \label{eq:dary_MPR}
    \cri_\nuser = \begin{cases} 1, & n = 0,1,\dots, \mpr \\
    \sum_{j=i}^{d_\text{min}} \cri_{I_j} , & n > \mpr 
    \end{cases}   
\end{align}
where $d_\text{min}$ is the minimum value of $o \in \{1,\dots, d\}$ for which it holds that
\begin{align}
\sum_{j=1}^{o} I_j \geq \nuser - \mpr.
\end{align}

Unfortunately, when $d>2$, the expressions \eqref{eq:dary_correct} and \eqref{eq:dary_MPR} can not be computed in the same manner as it can be done when $d = 2$.
In particular, the summands in \eqref{eq:dary_correct} and \eqref{eq:dary_MPR} are subject to the same recursion that holds for $\ecri_\nuser$, making the overall computation quickly intractable.
Further investigations with respect to this problem are out of the scope of this paper.
Instead,  we present some illustrative results obtained through a simulation-based study.

\begin{figure}[t]
  % Requires \usepackage{graphicx}
  \centering
 \includegraphics[width=0.65\columnwidth]{SIC.eps}
  %\includegraphics[width=\columnwidth]{SIC.eps}
  \caption{Throughput performance of $\tf$-ary tree-algorithms with \ac{SIC} as function of $d$, $\mpr =1$: red dots represent \ac{MST} results from~\cite{SICTA}, blue squares represent $\T_n$ obtained via simulations for $n=1000$. }
  \label{fig:sicta}
\end{figure}

Fig.~\ref{fig:sicta} compares the results for \ac{MST} with the gated access presented in~\cite{SICTA} with the ones for $\T_\nuser$ when $\nuser=1000$, obtained by averaging over 10000 simulation runs, wherein both cases it is assumed that the splitting is fair and that $\mpr=1$.
The latter can serve as a proxy for the MST for gated access for $K=1$, by considering that 
\begin{align}
\lim_{\nuser \rightarrow \infty} \T_n = \frac{1}{\lim_{\nuser \rightarrow \infty} \ecri_n / n}     
\end{align}
see Section~\ref{sec:gated}. %, we also note that there was no tangible difference in
Obviously, there is a huge difference among the two curves, which becomes more pronounced as $\tf$ increases.
The overall conclusion is that $\tf=2$ is the best choice, albeit with a much lower margin than the one in~\cite{SICTA}.

Finally, Fig.~\ref{fig:d-ary-sims} shows the conditional throughput $\T_\nuser$ for the combination of the splitting factor $\tf = \{ 3, 8\}$ and $\mpr \in \{1,4,16\}$; again, the results are obtained by averaging over 10000 simulation runs.
The already identified oscillatory behavior around the mean value (which are roughly 0.663 and 0.48 for $\tf=3$ and $\tf=8$, respectively; see also Fig.~\ref{fig:sicta}) is clearly present and the amplitude of the oscillations visibly amplifies with $\tf$ (also compare with with Fig.~\ref{fig:T}.
However, the analysis of this interesting phenomenon is out of the paper scope.

\begin{figure}[t]
  % Requires \usepackage{graphicx}
  \centering
  \includegraphics[width=0.65\columnwidth]{d-ary.eps}
  %\includegraphics[width=\columnwidth]{d-ary.eps}
  \caption{$\T_\nuser$ as function of $\nuser$ for $\tf \in \{ 3, 8\}$ and $\mpr \in \{1,4,16\}$. }
  \label{fig:d-ary-sims}
\end{figure}
